Random-sketching Techniques to Enhance the Numerical Stability of Block Orthogonalization Algorithms for s-step GMRES

We integrate random sketching techniques into block orthogonalization schemes needed for s-step GMRES. The resulting block orthogonalization schemes generate the basis vectors whose overall orthogonality error is bounded by machine precision as long as each of the corresponding block vectors are numerically full rank. We implement these randomized block orthogonalization schemes using standard distributed-memory linear algebra kernels for s-step GMRES available in the Trilinos software packages. Our performance results on the Perlmutter supercomputer (with four NVIDIA A100 GPUs per node) demonstrate that these randomized techniques can enhance the numerical stability of the orthogonalization and overall solver, without a significant increase in the execution time.

==> codes/2-stage-flat.tex <==
  \begin{algorithmic}[1]
  \Statex \textbf{Input:} $Q_{1:\ell-1}$, $V_{\ell:t}$
  \Statex \textbf{Output:}  $Q_{\ell:t}$ and $R_{1:t,k:t}$
  \State {\emph{// $t$ is last block column ID of the next big panel}}
  \State {\emph{// Orthogonalize new big panel against previous big panels}}
  \State [$\widehat{V}_j$, $R_{1:\ell-1,j}$] := BCGS($Q_{1:\ell-1}$,$V_j$)
  \State {\emph{// Intra-Big Panel PreProcess}}
  \State $t := \ell+\hat{s}/s-1$ 
  \For{$j = \ell, \ell+1, \dots, t$}
     \State [$\widehat{Q}_{j} $, $R_{\ell:j,j}$] := PreProc($\widehat{Q}_{\ell:j-1}$, $V_{j}$)
  \EndFor
  \State {\emph{// CholQR of big panel}}
  \State $T_{\ell:t,\ell:t} : = \mbox{CholQR}(\widehat{Q}_{\ell:t})$
  \State $R_{\ell:t,\ell:t} := T_{\ell:t,\ell:t} R_{\ell:t,\ell:t}$
  \State {\emph{// Orthogonalization}}
   \State [$Q_{\ell:t}, T_{1:t,\ell:t}$] = BCGS+CholQR($Q_{1:\ell-1}$, $Q_{\ell:t}$)
   \State $R_{1:\ell-1,\ell:t} := T_{1:\ell-1,\ell:t}R_{\ell:t,\ell:t} + R_{1:\ell-1,\ell:t}$
   \State $R_{\ell:t,\ell:t} := T_{\ell:t,\ell:t} R_{\ell:t,\ell:t}$
  \end{algorithmic}

==> codes/2stage-random.tex <==
  \begin{algorithmic}[1]
  \Statex \textbf{Input:} $Q_{1:j_1-1}$ and $V_{j_1:j_2}$
  \Statex \textbf{Output:}  $Q_{j_1:j_2}$ and $R_{1:j_2,j_1:j_2}$
        \State\emph{// First inter big-panel ortho}
        \State [$\widehat{V}_{j_1:j_2}$, $\widehat{R}_{1:j_1-1,j_1:j_2}$] := BCGS($Q_{1:j_1-1}$, $V_{j_1:j_2}$)
        \State\emph{// First intra big-panel ortho}
        \State [$\widetilde{V}_{j_1:j_2}$, $\widehat{R}_{j_1:j_2,j_1:j_2}$] := incRandQR($\widehat{V}_{j_1:j_2}$)
        \State [$\widehat{Q}_{j_1:j_2}$, $\widehat{T}_{j_1:j_2,j_1:j_2}$] := CholQR($\widetilde{V}_{j_1:j_2}$)
        \State $\widehat{R}_{j_1:j_2,j_1:j_2} := \widehat{T}_{j_1:j_2,j_1:j_2}\widehat{R}_{j_1:j_2,j_1:j_2}$
        \\
        \State\emph{// Second inter big-panel ortho}
        \State [$Q_{j_1:j_2}$, $T_{1:j_1-1,j_1:j_2}$] := BCGS($Q_{1:j_1-1}$, $\widehat{Q}_{j_1:j_2}$)
        \State\emph{// Second intra big-panel ortho}
        \State [$Q_{j_1:j_2}$, $T_{j_1:j_2,j_1:j_2}$] := CholQR($Q_{j_1:j_2}$)
        \State\emph{// Update $R_{1:j_2,j_1:j_2}$}
        \State $R_{1:j_1-1,j_1:j_2} := \widehat{R}_{1:j_1-1,j_1:j_2} + \widehat{T}_{j_1:j_2,j_1:j_2}\widehat{R}_{j_1:j_2,j_1:j_2}$ 
        \State $R_{j_1:j_2,j_1:j_2} := T_{j_1:j_2,j_1:j_2} \widehat{R}_{j_1:j_2,j_1:j_2}$
  \end{algorithmic}
  

==> codes/bcgs2-rand.tex <==
  \begin{algorithmic}[1]
  \Statex \textbf{Input:} $Q_{1:j-1}$ and $V_j$
  \Statex \textbf{Output:}  $Q_j$ and $R_{1:j-1,j}$
        \State {\emph{// BCGS orthogonalization}}
        \State [$\widehat{V}_j$, $\widehat{R}_{1:j-1,j}$] := BCGS($Q_{1:j-1}$, $V_{j}$)
        \State [$\widehat{Q}_j$, $\widehat{R}_{j,j}$] := RandCholQR($\widehat{V}_{j}$)
        \If {$j > 1$}
          \State {\emph{// BCGS re-orthogonalization}}
          \State [$Q_j$, $T_{1:j-1,j}$] := BCGS($Q_{1:j-1}$,  $\widehat{Q}_{j}$)
          \State [$Q_j$, $T_{j,j}$] := CholQR($Q_{j}$)
          \State{\emph{// Update upper-triangular matrix}}
          \State $R_{1:j-1,j} := R_{1:j-1,j} + T_{1:j-1,j}\widehat{R}_{j,j}$
          \State $R_{j,j} := T_{j,j}\widehat{R}_{j,j}$
        \EndIf
  \end{algorithmic}

==> codes/cholQR2.tex <==
  \begin{algorithmic}[1]
      \Statex \textbf{Input:}  $\widehat{V}_j \in \mathbb{R}^{n\times s}$
      \Statex \textbf{Output:} $Q_j \in \mathbb{R}^{n\times s}$, $R_{j,j} \in \mathbb{R}^{s \times s}$
        \State {\emph{// CholQR orthogonalization}}
        \State [$\widehat{Q}_j$, $R_{j,j}$] := CholQR($\widehat{V}_j$)
        \State {\emph{// CholQR re-orthogonalization}}
        \State [$Q_j$, $T_{j,j}$] := CholQR($\widehat{Q}_j$)
        \State{\emph{// Update upper-triangular matrix}}
        \State $R_{j,j} := T_{j,j}R_{j,j}$
  \end{algorithmic}

==> codes/gmres.tex <==
%\begin{algorithm}
  \begin{algorithmic}[1]
  \Statex \textbf{Input:}  coefficient matrix $A$, right-hand-side vector $b$, initial vector $x$,  and appropriately-chosen ``change-of-basis-matrix'' $T$
          (see \cite[Section 3.2.3]{Hoemmen:2010} for details)
  \Statex \textbf{Output:}  approximate solution $x$
    \State $r = b-Ax$,
    \While {not converged}
      \State $r_{1,1} = r/\|r\|_2$    
      \State $q_1 = r/r_{1,1}$
      \For{$j=1:m$}
        \State{\emph{// SpMV, combined with preconditioner}}
          \State $v_{j+1} = AM^{-1} q_{j}$
        \State{\emph{// Orthogonalization}}
        \State $[q_{j+1}, r_{j+1}] := \mbox{Orth}(Q_{1:(j-1)}, v_{j+1})$
      \EndFor
      \State{\emph{// Generate the Hessenberg matrix s.t. $AQ = QH$}}
      \State $H_{1:m+1,1:m} = R_{1:m+1,1:m+1} T R_{1:m,1:m}^{-1}$
      \State{\emph{// Compute approximate solution}}
      \State{\emph{// \;with minimum residual}}
      \State $\hat{y} = \argmin_{y\in Q_{1:m+1}} \|{\gamma e_1 - H_{1:m+1,1:m} y}\|_2$
      \State $x = x + V_m\hat{y}$
      \State $r = b - Ax$ %If $\|{r_m}\|_2/\|{r_0}\|_2 \le rTol$, stop. Else, set $x_0 = x_m$, $r_0 = r_m$ and go to Step 2.
    \EndWhile
  \end{algorithmic}
%\end{algorithm}

==> codes/incCholQR.tex <==
  \begin{algorithmic}[1]
      \Statex \textbf{Input:}  $\widehat{Q}_{\ell:j-1}$, $\widehat{V}_{j}$
      \Statex \textbf{Output:} $\widehat{Q}_{j}$, $R_{1:j,j}$
      %\For{$\hat{j}=j_1,\dots,j_2$}
             \State{\emph{// Orthogonalize against previous blocks (within big panel)}}
             \State $R_{\ell:j-1,j} := Q_{\ell:j-1}^T V_j$ \hspace{.5cm}
                    {\scriptsize (i.e., $R_{j,k} = G_{j,k} - \sum_{i:k-1} R_{i,j}^T R_{i,k}$)}
             \State $\widehat{Q}_j := \widehat{V}_j - \widehat{P}Q_{\ell:j-1} R_{\ell:j-1,j}$
             \State{\emph{// Orthogonalize the block}}
             \State  {$[\widehat{Q}_j,R_{j,j}] := \mbox{CholQR}(\widehat{Q}_{j})$ \hspace{.2cm}
                     {\scriptsize (i.e., $R_{j,j} = \mbox{chol}(G_{j,j}-\sum_{i:j-1} R_{i,j}^T R_{i,j}$)}}
      %\EndFor
  \end{algorithmic}

==> codes/precond.tex <==
  \begin{algorithmic}[1]
  \Statex \textbf{Input:}  $Q_{1:\ell-1}$, $\widehat{Q}_{\ell:j-1}$, $V_j$
  \Statex \textbf{Output:} $\widehat{Q}_j$ and $R_{1:j,j}$
     \State {\emph{// Orthogonalize against previous big panels}}
     \State [$\widehat{V}_{j}$, $R_{1:\ell-1,j}$] := BCGS($Q_{1:\ell-1}$, $V_{j}$)
     \State {\emph{// Preprocess current panel (within current big panel)}}
     \State [$\widehat{Q}_{j}$, $R_{j,j}$] := Intra-PreProc($\widehat{Q}_{\ell:j-1}$, $\widehat{V}_{j}$)
  \end{algorithmic}
